Data-Driven Gain Scheduling Control of Linear Parameter-Varying Systems using Quadratic Matrix Inequalities

This paper synthesizes a gain-scheduled controller to stabilize all possible Linear Parameter-Varying (LPV) plants that are consistent with measured input/state data records. Inspired by prior work in data informativity and LTI stabilization, a set of Quadratic Matrix Inequalities is developed to represent the noise set, the class of consistent LPV plants, and the class of stabilizable plants. The bilinearity between unknown plants and `for all' parameters is avoided by vertex enumeration of the parameter set. Effectiveness and computational tractability of this method is demonstrated on example systems.

==> sections/continuous_time.tex <==
\section{Continuous-Time}

We briefly consider the case where the \ac{LPVA} system \eqref{eq:LPVA} is in continuous-time , and the data $\dc$ is a collection 

==> sections/h2_control.tex <==
\section{H2 Optimal Control}
\label{sec:h2_control}

A discrete-time LPVA state-space system with external input $\rev{\xi} \in \R^{e}$  and regulated output $z \in \R^r$ given matrices $C \in \R^{r \times n}, \ D \in \R^{r \times m}, F \in \R^{n \times e}$ is
\begin{align}
    x^+ &= \textstyle \sum_{\ell=1}^L \theta_\ell A_\ell x + B u + F \rev{\xi}, &     z &= C x + Du. \label{eq:h2_sys}
\end{align}

\rev{The recorded data in $\dc$ has $\rev{\xi}=0$ while $\mathbf{W} \in \qbp{\Phi}$. The input $\rev{\xi}$ is applied during system execution.}

% Let $\delta_{k,o}$ be an impulse applied to coordinate $k$ for $k=1..e$. 
Define the $\rev{H}_2$ norm of  \eqref{eq:h2_sys} as \rev{
% as the worst case (over all parameter trajectories) expected value of the output energy $\norm{z}_2^2$ to an \MS{impulsive input $w(t)=w*\delta(t)$ with $\mathcal{E}(ww^T)=I$.}
the worst-case (over all parameter trajectories) expected root-mean-square value of $\norm{z}_2$  when the input $\xi$ is a white noise process with identity covariance.
}
Then we have the following bound:
%Define the $\mathcal{H}_2$ norm of  \eqref{eq:h2_sys} as the worst case value of $\norm{z}_2$ over all parameter trajectories $\theta(0)..\theta(T-1)$ and mixed impulse-inputs $\rev{\xi}(0) = q, \ \rev{\xi}(1)=0\ldots \rev{\xi}(T-1) = 0$ with $q \in \R_{\geq 0}^e, \ \sum_{k=1}^{e} w_k = 1$.
% Define the $\mathcal{H}_2$ norm of  \eqref{eq:h2_sys} as the worst case, over all parameter trajectories, of $\|z\|_2$ when $\rev{\xi} = \delta_{k,o}$. Then we have the following bound:
% The following \ac{LMI} to minimize the $H_2$-norm between $\rev{\xi} \rightarrow z$ is expressed in Section 4.2.2 of \cite{caverly2019lmi}.
% \urg{It is suggested to use the following instead of above, since it contains the smallest size of Gram matrix and directly corresponds to your algorithm. It is fine that $E$ is bilinear since it is assumed known. A few changes: a) I use $Y,M$ instead of $P,F$ to be consistent with other parts. b) replace $\nu$ by $\gamma$ to avoid confusion. c) size of $Z$ is r. d) modify the problem to be worst-case $H_2$ control.
\begin{prop}
\label{prob:h2_single}\rev{There exists a gain-scheduled controller $u = K(\theta) x$ such that the closed-loop}  $H_2$ norm of \rev{the LPVA system} \eqref{eq:h2_sys} is bounded above by $\gamma \in \R_+$ if \rev{for all $v=1..N_v$} the following \ac{LMI} is feasible
%\rev{discrete-time version of }
\begin{subequations}
\label{eq:h2_single}
\begin{align}
    \find_{P, Z, S} \quad & \begin{bmatrix} P - F F^T & A_v P + B S_v \\ \ast & P \label{eq:h2_single_schur}\end{bmatrix} \in \psd_{++}^{2n} \\
    & \begin{bmatrix} Z & C P + D S_v \\ \ast & P \end{bmatrix} \in \psd_{++}^{n+r}  \label{eq:h2_z}\\
    & \Tr Z \leq \gamma^2 \\
    & P \in \psd^n_{++}, \ Z \in \psd^r_+, \ S_v \in \R^{m \times n} \label{eq:h2_def}.
\end{align}
\end{subequations}
The gain-scheduled controller $K(\theta)$ may be recovered from $\{\rev{\forall v: \ }K_v = S_v P^{-1}\}$ and \rev{Eq. \eqref{eq:gain_sched}}.
\end{prop} 
The matrix variables $(Z, P)$ and given entries $(C, D, F)$ are independent of $(A, B) \in \Sigma_\dc$.
The indexing matrix $E_0$ may be defined as
$E_0 = [I_n, \0_{n \times (n(L+2)+m)}]^T$
in order to pose the following LMI at each vertex $v$
\begin{equation}
\label{eq:h2_lmi_gamma}
    \Gamma_v(\beta_v) - E_0 F F^T E_0^T- \alpha_v \begin{bmatrix}\Psi & \0 \\ \0 & \0_{n\times n}\end{bmatrix} \in \psd_{+}^{n(L+2)+m}. 
\end{equation}

Constraint \eqref{eq:h2_lmi_gamma} is equal to \eqref{eq:gamma_bv_lmi} when $F = \0_{n\times e}$, given that conditions \eqref{eq:h2_single_schur} and \eqref{eq:lpv_stab_noiseless_kv} are identical under this restriction.


Worst-case $H_2$ control of \eqref{eq:h2_sys} for all $(A(\theta), B) \in \Sigma_\dc$ given $(C, D, F)$ may be conducted by solving
\begin{subequations}
\label{eq:lpv_qmi_h2}
\begin{align}
  \rev{\gamma^2 =} \inf & \quad  \Tr{Z} \\
  & P \in \psd_{++}^n, \ Z \in \psd_+^r \label{eq:lpv_qmi_alg_p_h2}\\
    & \alpha \in \R_{\geq 0}^{N_v}, \ \beta \in \R_{> 0}^{N_v}, \\
    & \textrm{LMIs \eqref{eq:h2_z} and \eqref{eq:h2_lmi_gamma} hold}  & & \forall v = 1..N_v \label{eq:lpv_qmi_alg_gamma_h2}
\end{align}
\end{subequations}
% \MS{This is not the resulting $H_2$ norm, it is an upper bound, right?. Should say. Using the gain scheduled control matrices $\{K_v = S_v P^{-1}\}_{v=1}^{N_v}$ leads to a closed loop system with $H_2$ norm bounded above by $\gamma = \sqrt{\Tr{Z}}$ }
\rev{The resultant $H_2$ norm is upper-bounded by $\gamma = \sqrt{\Tr{Z}}$ when using gain-scheduled control matrices $\{K_v = S_v P^{-1}\}_{v=1}^{N_v}$.}
All results in this section may be extended to continuous-time $H_2$ control with appropriate \acp{LMI} \cite{zhou1998essentials}.
% \begin{algorithm}[h]
% \caption{LPV $H_2$-optimal Control Generation}\label{alg:lpv_qmi_h2}
% \KwIn{Data $\dc$,  Noise description $\Phi$, Vertices $\Omega$, Design Matrices $(C, D, F)$}
% \KwOut{ Vertex-parameterized controls $\{K_v\}$ }
% % $K \in \R^{n \times m}, \ M \in (\R[,B,\dx])^{n \times n}_{\leq 2d}$ \
% Solve or return an infeasibility certificate, 
% \begin{subequations}
% \label{eq:lpv_qmi_h2}
% \begin{align}
%   \inf & \quad  \Tr{Z} \\
%   & P \in \psd_{++}^n, \ Z \in \psd_+^r \label{eq:lpv_qmi_alg_p_h2}\\
%     & \alpha \in \R_{\geq 0}^{N_v}, \ \beta \in \R_{> 0}^{N_v}, \\
%     & \textrm{LMIs \eqref{eq:h2_z} and \eqref{eq:h2_lmi_gamma} hold}  & & \forall v = 1..N_v \label{eq:lpv_qmi_alg_gamma_h2}
% \end{align}
% \end{subequations}\\
% Return $\gamma = \sqrt{\Tr{Z}}, \ \{K_v = S_v P^{-1}\}_{v=1}^{N_v}$
% \end{algorithm}

% when $D = 0$ \urg{TODO: is this correct?}.

% \urg{Code $H_2$ and run experiment}



% \urg{Based on Section V of \cite{waarde2020noisy}. I need to implement this.}

% \urg{There may not be room for $H_2$ control in the 6-page LCSS format. This could be saved for the ArXiv copy. However, that's not enough for a full-fledged journal version.}
